The Star Formation History of the Large Magellanic Cloud

We present the first-ever global, spatially-resolved reconstruction of the star formation history (SFH) of the Large Magellanic Cloud (LMC), based on the application of our StarFISH analysis software to the multiband photometry of twenty million of its stars from the Magellanic Clouds Photometric Survey. The general outlines of our results are consistent with previously published results: following an initial burst of star formation, there was a quiescent epoch from approximately 12 to 5 Gyr ago. Star formation then resumed and has proceeded until the current time at an average rate of roughly 0.2 solar masses/yr, with temporal variations at the factor-of-two level. The re-ignition of star formation about 5 Gyr ago, in both the LMC and SMC, is suggestive of a dramatic event at that time in the Magellanic system. Among the global variations in the recent star formation rate are peaks at roughly 2 Gyr, 500 Myr, 100 Myr and 12 Myr. The peaks at 500 Myr and 2 Gyr are nearly coincident with similar peaks in the SFH of the Small Magellanic Cloud, suggesting a joint history for these galaxies extending back at least several Gyr. The chemical enrichment history recovered from our StarFISH analysis is in broad agreement with that inferred from the LMC's star cluster population, although our constraints on the ancient chemical enrichment history are weak. We conclude from the concordance between the star formation and chemical enrichment histories of the field and cluster populations that the field and cluster star formation modes are tightly coupled.

==> ast.tex <==
%Table of AST regions
\begin{deluxetable}{rrrr}
\tablecaption{The Artificial Stars Tests \label{tab:ast}}
\tablewidth{0pt}
\tablehead{ 
  \colhead{Subregion\tnm{a}} & 
  \colhead{$N_\star/\Box\arcmin$} & 
  \colhead{$\langle A_V(hot) \rangle$ [mag]} & 
  \colhead{$\langle A_v(cool) \rangle$ [mag]} 
}
\startdata
DP &  47.4 & 0.7  & 0.4 \\
EP &  69.4 & 0.7  & 0.4 \\
CF &  70.9 & 0.7  & 0.6 \\
JC &  77.7 & 0.6  & 0.5 \\
GC &  79.0 & 0.5  & 0.5 \\
FP &  94.3 & 0.5  & 0.4 \\
EF & 105.3 & 0.6  & 0.5 \\
KC & 105.9 & 0.7  & 0.5 \\
LC & 125.7 & 0.6  & 0.5 \\
PN & 131.2 & 0.4  & 0.4 \\
MN & 142.9 & 0.4  & 0.4 \\
ON & 145.9 & 0.25 & 0.4 \\
NN & 160.7 & 0.2  & 0.3 \\
KF & 174.6 & 0.5  & 0.4 \\
HF & 181.0 & 0.5  & 0.4 \\
IF & 186.7 & 0.5  & 0.4 \\
OF & 221.1 & 0.4  & 0.3 \\
PD & 174.6 & 0.7  & 0.5 \\
PI & 142.9 & 0.8  & 0.7 \\
PM & 131.2 & 0.5  & 0.5 \\
\enddata
\tablenotetext{a}{Each two-letter code indicates the region's position
in our gridding of the LMC (see Figure~\ref{fig:datagrid}).}
\end{deluxetable}


==> cluster_agez.tex <==
%Table of LMC Cluster Ages and Metallicities from the literature
\begin{deluxetable}{rrrrrrl}
\tablecaption{LMC Cluster Ages and Metallicities \label{tab:cluster_agez}}
\tablewidth{0pt}
\tablehead{ 
  \colhead{Cluster} & 
  \colhead{[Fe/H]} & \colhead{$\sigma_{[Fe/H]}$} &
  \colhead{log(Age)} & \colhead{$\sigma_{log(Age)}$} &
  \colhead{Reference} & \colhead{Notes}
}
\startdata
Reticulum & $-$1.66 & 0.12 & 10.13 &  0.05 & \cite{mac04}  & {a}  \\
BRHTb     & $-$0.40 & 0.0  &  8.0  &  0.0  & \cite{pia03}  & {bc} \\
ESO121    & $-$0.97 & 0.1  &  9.96 &  0.04 & \cite{mac06}  & \nodata  \\
R136      & $-$0.4  & 0.0  &  7.0  &  0.0  & \cite{hun95}  & {bc} \\
OHSC33    & $-$1.05 & 0.2  &  9.18 &  0.03 & \cite{bic98}  & \nodata  \\
OHSC37    & $-$0.7  & 0.2  &  9.32 &  0.03 & \cite{bic98}  & \nodata  \\
Hodge11   & $-$1.84 & 0.0  & 10.13 &  0.05 & \cite{gro06}  & {ad} \\
LH47/48   & $-$0.4  & 0.0  &  6.3  &  0.0  & \cite{om95}   & {bc} \\
LH52/53   & $-$0.4  & 0.0  &  7.0  &  0.0  & \cite{hill95} & {bc} \\
LH72      & $-$0.6  & 0.0  &  6.95 &  0.25 & \cite{ols97}  & {b}  \\
LH77      & $-$0.4  & 0.0  &  7.20 &  0.14 & \cite{dh98}   & {b}  \\
LW224     &  0.0  & 0.2  &  8.85 &  0.0  & \cite{pia03}  & {c}  \\
SL8       & $-$0.55 & 0.2  &  9.26 &  0.03 & \cite{bic98}  & \nodata  \\
SL126     & $-$0.5  & 0.2  &  9.34 &  0.03 & \cite{bic98}  & \nodata  \\
SL218     & $-$0.40 & 0.0  &  7.70 &  0.0  & \cite{pia03}  & \nodata  \\
SL244     & $-$0.7  & 0.2  &  9.11 &  0.09 & \cite{gei03}  & {e}  \\
SL262     & $-$0.6  & 0.2  &  9.32 &  0.03 & \cite{bic98}  & \nodata  \\
SL359     & $-$0.4  & 0.2  &  9.20 &  0.1  & \cite{gei03}  & \nodata  \\
SL388     & $-$0.39 & 0.05 &  9.34 &  0.03 & \cite{gro06}  & {f}  \\
SL444     & $-$0.4  & 0.2  &  8.7  &  0.0  & \cite{pia03}  & {c}  \\
SL446A    & $-$0.9  & 0.2  &  9.34 &  0.1  & \cite{gei03}  & \nodata  \\
SL451     & $-$0.75 & 0.2  &  9.34 &  0.03 & \cite{bic98}  & \nodata  \\
SL503     & $-$0.4  & 0.0  &  7.20 &  0.22 & \cite{dh98}   & {b}  \\
SL505     & $-$0.5  & 0.2  &  8.95 &  0.09 & \cite{gei03}  & \nodata  \\
SL506     & $-$0.45 & 0.1  &  9.35 &  0.03 & \cite{ker07}  & \nodata  \\
SL509     & $-$0.65 & 0.0  &  9.08 &  0.0  & \cite{pia03}  & {bc} \\
SL548     &  0.0  & 0.2  &  8.60 &  0.0  & \cite{pia03}  & {c}  \\
SL549     & $-$0.9  & 0.2  &  9.30 &  0.1  & \cite{gei03}  & \nodata  \\
SL555     & $-$0.7  & 0.2  &  9.20 &  0.12 & \cite{gei03}  & \nodata  \\
SL556     & $-$0.7  & 0.2  &  9.32 &  0.0  & \cite{woo03}  & {c}  \\
SL663     & $-$0.7  & 0.1  &  9.50 &  0.05 & \cite{ker07}  & {e}  \\
SL674     & $-$0.9  & 0.2  &  9.30 &  0.08 & \cite{gei03}  & \nodata  \\
SL678     & $-$0.8  & 0.2  &  9.18 &  0.08 & \cite{gei03}  & \nodata  \\
SL769     & $-$0.35 & 0.0  &  9.26 &  0.0  & \cite{pia03}  & {bc} \\
SL817     & $-$0.55 & 0.2  &  9.18 &  0.03 & \cite{bic98}  & \nodata  \\
SL842     & $-$0.65 & 0.2  &  9.34 &  0.03 & \cite{bic98}  & \nodata  \\
SL862     & $-$0.9  & 0.2  &  9.26 &  0.03 & \cite{bic98}  & \nodata  \\
SL896     & $-$0.6  & 0.2  &  9.36 &  0.09 & \cite{pia02}  & \nodata  \\
NGC1651   & $-$0.53 & 0.03 &  9.30 &  0.03 & \cite{gro06}  & {eg} \\
NGC1711   & $-$0.57 & 0.17 &  7.7  &  0.05 & \cite{dir00}  & \nodata  \\
NGC1718   & $-$0.4  & 0.1  &  9.31 &  0.03 & \cite{ker07}  & {e}  \\
NGC1754   & $-$1.42 & 0.15 & 10.19 &  0.06 & \cite{ols98}  & \nodata  \\
NGC1777   & $-$0.6  & 0.1  &  9.06 &  0.04 & \cite{ker07}  & \nodata  \\
NGC1786   & $-$2.1  & 0.3  & 10.13 &  0.1  & \cite{bro96}  & {h}  \\
NGC1806   & $-$0.71 & 0.23 &  8.7  &  0.1  & \cite{dir00}  & \nodata  \\
NGC1831   & $-$0.1  & 0.1  &  8.85 &  0.05 & \cite{ker07}  & \nodata  \\
NGC1835   & $-$1.62 & 0.15 & 10.21 &  0.07 & \cite{ols98}  & \nodata  \\
NGC1836   &  0.0  & 0.2  &  8.60 &  0.0  & \cite{pia03}  & {c}  \\
NGC1838   & $-$0.4  & 0.0  &  8.0  &  0.0  & \cite{pia03}  & {bc} \\
NGC1839   & $-$0.4  & 0.0  &  8.10 &  0.0  & \cite{pia03}  & {bc} \\
NGC1841   & $-$2.02 & 0.02 & 10.13 &  0.1  & \cite{gro06}  & {ai} \\
NGC1846   & $-$0.40 & 0.0  &  9.3  &  0.03 & \cite{mac07}  & {b}  \\
NGC1850A  & $-$0.12 & 0.03 &  7.7  &  0.1  & \cite{gil94}  & \nodata  \\
NGC1850B  & $-$0.12 & 0.03 &  6.6  &  0.1  & \cite{gil94}  & \nodata  \\
NGC1856   & $-$0.4  & 0.1  &  8.47 &  0.04 & \cite{ker07}  & \nodata  \\
NGC1858   & $-$0.4  & 0.0  &  6.9  &  0.0  & \cite{val94b} & {bc} \\
NGC1860   &  0.0  & 0.2  &  8.4  &  0.0  & \cite{pia03}  & {c}  \\
NGC1863   & $-$0.40 & 0.0  &  7.7  &  0.0  & \cite{pia03}  & {bc} \\
NGC1865   & $-$0.2  & 0.2  &  8.7  &  0.0  & \cite{pia03}  & {c}  \\
NGC1866   & $-$0.43 & 0.18 &  8.0  &  0.0  & \cite{hil95}  & {c}  \\
NGC1868   & $-$0.7  & 0.1  &  9.05 &  0.03 & \cite{ker07}  & \nodata  \\
NGC1898   & $-$1.37 & 0.15 & 10.13 &  0.07 & \cite{ols98}  & \nodata  \\
NGC1928   & $-$1.27 & 0.14 & 10.13 &  0.1  & \cite{mac04}  & {a}  \\
NGC1939   & $-$2.10 & 0.19 & 10.13 &  0.1  & \cite{mac04}  & {a}  \\
NGC1948   & $-$0.4  & 0.0  &  6.85 &  0.15 & \cite{wil96}  & {b}  \\
NGC1955   & $-$0.4  & 0.0  &  7.19 &  0.15 & \cite{dh98}   & {b}  \\
NGC1978   & $-$0.38 & 0.07 &  9.54 &  0.0  & \cite{fer06}  & {ce} \\
NGC2004   & $-$0.4  & 0.0  &  7.19 &  0.15 & \cite{dh98}   & {be} \\
NGC2005   & $-$1.35 & 0.15 & 10.22 &  0.11 & \cite{ols98}  & \nodata  \\
NGC2019   & $-$1.23 & 0.15 & 10.21 &  0.08 & \cite{ols98}  & \nodata  \\
NGC2027   & $-$0.4  & 0.0  &  7.06 &  0.14 & \cite{dh98}   & {b}  \\
NGC2031   & $-$0.52 & 0.21 &  8.2  &  0.1  & \cite{dir00}  & \nodata  \\
NGC2121   & $-$0.4  & 0.1  &  9.46 &  0.07 & \cite{ker07}  & {e}  \\
NGC2134   & $-$0.4  & 0.0  &  8.28 &  0.0  & \cite{val94a} & {bc} \\
NGC2136   & $-$0.55 & 0.23 &  8.0  &  0.1  & \cite{dir00}  & \nodata  \\
NGC2155   & $-$0.7  & 0.1  &  9.48 &  0.03 & \cite{ker07}  & {e}  \\
NGC2162   & $-$0.4  & 0.1  &  9.10 &  0.03 & \cite{ker07}  & \nodata  \\
NGC2164   & $-$0.2  & 0.2  &  8.0  &  0.0  & \cite{sr91}   & {c}  \\
NGC2173   & $-$0.6  & 0.1  &  9.21 &  0.04 & \cite{ker07}  & {e}  \\
NGC2209   & $-$0.5  & 0.1  &  9.08 &  0.03 & \cite{ker07}  & \nodata  \\
NGC2210   & $-$1.75 & 0.1  & 10.13 &  0.1  & \cite{hill00} & {ehi}\\
NGC2213   & $-$0.7  & 0.1  &  9.23 &  0.04 & \cite{ker07}  & {e}  \\
NGC2214   & $-$0.2  & 0.2  &  8.0  &  0.0  & \cite{sr91}   & {c}  \\
NGC2249   & $-$0.45 & 0.1  &  9.35 &  0.03 & \cite{ker07}  & \nodata  \\
NGC2257   & $-$1.63 & 0.21 & 10.2  &  0.1  & \cite{dir00}  & \nodata  \\
\enddata

\tablenotetext{a}{age found to be ``equal to M92''; age error is our
  estimate from isochrones}
\tablenotetext{b}{no [Fe/H] error given}
\tablenotetext{c}{no age error given}
\tablenotetext{d}{age reference: \cite{joh99}}
\tablenotetext{e}{discrepant [Fe/H] measurements exist in literature}
\tablenotetext{f}{age reference: \cite{bic98}}
\tablenotetext{g}{age reference: \cite{ker07}}
\tablenotetext{h}{age found to be ``equal to M68''; age error is our 
  estimate from isochrones}
\tablenotetext{i}{age reference: \cite{bro96}}

\end{deluxetable}


==> figures.tex <==
%CMD triptych for entire LMC population
\begin{figure}[htbp]
\epsscale{0.7}
\plotone{figure1.eps}
\caption{A ``CMD triptych'' illustrating our $UBVI$ photometry of
  $\sim$20 million LMC stars.  Each CMD panel is a Hess diagram whose
  pixel values are proportional to the number of stars in each pixel.
  The mixed populations evident in these CMDs represent a ``fossil
  record'' of a complex star-formation history in this
  galaxy. \label{fig:cmds} }
\end{figure}

% extinction distros from selected regions
\begin{figure}[htbp]
\plotone{figure2.eps}
\caption{Extinction distributions for both hot (unshaded line) and
  cool (shaded line) star samples, for eight small subregions sampling
  various substructures in the LMC, as labeled in each panel.  The
  plot illustrates the spatial variability in the extinction
  properties, as well as the wide distribution of extinction values
  within many of the regions. Derived negative extinctions arise due
  to photometric errors \cite[see][for more details]{zar04} and 
  such values are set to $A_V = 0$. \label{fig:extdist} }
\end{figure}

% CMDs from select regions to illustrate spatial variation in 
% stellar pops and crowding conditions
\begin{figure}[htbp]
\plotone{figure3.eps}
\caption{$B-V$ color-magnitude diagrams for the same eight LMC
  subregions as shown in Figure~\ref{fig:extdist}.  Stars brighter
  than $V$=16~mag are shown with a larger point, to reveal the sparse
  distribution of these objects.  The dramatic spatial variation in
  the stellar populations evident in this plot motivates a
  comprehensive, spatially-resolved analysis of the LMC's
  SFH. \label{fig:cmdsample} }
\end{figure}

% stellar density map, with hierarchical grid
\begin{figure}[htbp]
\plotone{figure4.eps}
\caption{A stellar flux density map derived from our $BVI$ photometry
  of the LMC.  Overplotted on this map, we show our gridding strategy
  for reconstructing the spatially-resolved SFH.  We divide the MCPS
  region into $24^\prime\times24^\prime$ cells.  Each of these cells
  may be further subdivided into a 2x2 grid of subregions, if the
  number of stars in the cell exceeds a threshold value.  In
  practice, most of the top-level grid cells are subdivided in this
  way. \label{fig:datagrid} }
\end{figure}

% Gridding strategy for the CMDs for StarFISH analysis
\begin{figure}[htbp]
\epsscale{0.5}
\plotone{figure5.eps}
\caption{Gridding strategy for the $B-V$ and $V-I$ CMD planes, for our
  StarFISH analysis.  The grid emphasizes the luminosity function of
  the main sequence (green boxes), the red giant branch and red clump
  (black boxes), and the red and blue supergiant sequences (red and
  blue boxes, respectively). \label{fig:cmdgrid} }
\end{figure}

% Map of subregions given special attention
\begin{figure}[htbp]
\epsscale{1.0}
\plotone{figure6.eps}
\caption{A star-count map of the LMC, in which the pixel value in each
  grid region is proportional to the number of stars present in that
  region.  The map highlights several collections of regions for which
  we will examine the SFH in detail: the LMC Bar (red), the Outer Bar
  (orange), 30~Doradus (magenta), the ``Southeast Arm'' (green), the
  ``Northwest Arm'' (cyan), the ``Blue Arm'' (blue), Constellation~III
  (pink), and the ``Northwest Void'' (yellow).
\label{fig:regmap} }
\end{figure}

\clearpage

% SFH results for HST studies of Bar fields
\begin{figure}[htbp]
\plotone{figure7.eps}
\caption{The SFH solutions for ages $>4$~Gyr from three independent
  studies of the LMC Bar, using HST imaging.  The solutions are:
  \cite{ols99} (red line), \cite{hol99} (green line), and \cite{sh02}
  (blue line).  The three solutions show remarkable agreement,
  especially when considering that \citeauthor{ols99} chose a
  relatively young age limit of 10~Gyr.  In the present analysis, we
  will require that our SFH solutions conform to the black curve for
  ages older than 4~Gyr.  In this way, we rely on the deep HST imaging
  to supplement our relatively shallow ground-based
  data. \label{fig:hstsfh} }
\end{figure}

%Sample SFH solution for a particular LMC region
%\begin{figure}[htbp]
%\epsfig{figure=sfhsample.eps,width=5in,angle=-90}
%\caption{A sample StarFISH solution for a particular LMC subregion in
%  the northern disk of the LMC.  The time axis is shown with a linear
%  scale that is broken into three segments: the left panel covers
%  $\sim$100~Myr, the middle panel covers $\sim$1~Gyr, and the right
%  panel covers $\sim$14~Gyr.  The best-fit star formation rate (SFR)
%  as a function of age is shown with a thick black line; the
%  uncertainty on the fit (including covariance between age bins) is
%  shown as a grey shaded envelope.  The distribution of metallicity at
%  each age is shown by the mix of colors below the SFR line (Z=0.001
%  in blue; Z=0.0025 in green; Z=0.004 in yellow; Z=0.008 in
% red). \label{fig:sfhsample} }
%\end{figure}

% map of the LMC's SFH
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure8.eps}
\caption{The map of the LMC's SFH, based on the StarFISH solutions for
  over 1300 subregions.  The pixel value for each region is
  proportional to the star formation rate at that location, color
  coded for the metallicity (with Z=0.001 shown as blue, Z=0.004 shown
  as green, and Z=0.008 shown as red).  There is no color-coding for
  log(Age)$<8.0$, because the fitter is not given multiple metallicity
  bins for these young ages.\label{fig:sfhmap} }
\end{figure}

% map of the LMC's SFH, expressed as stellar mass formed per timestep
\begin{figure}[htbp]
\epsscale{0.85} \plotone{figure9.eps}
\caption{The map of the LMC's SFH, based on the StarFISH solutions for
  over 1300 subregions. In this version of the map, the pixel values
  are proportional to the total stellar mass formed, rather than the
  star formation rate.\label{fig:sfhmap_stellarmass} }
\end{figure}

% correlation of young SF activity with Halpha
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure10.eps}
\caption{The correlation of the recent (Age $<12.5 $~Myr) star-formation
  activity in the LMC based on our analysis, with the H$\alpha$ image
  of the LMC from the Magellanic Clouds Emission Line Survey (MCELS)
  \citep{poi08}. \label{fig:youngmap} }
\end{figure}

% total SFH for the LMC
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure11.eps}
\caption{The total SFH of the LMC, computed by summing over all 1376
  regions covering the MCPS survey region. 
   The time axis is shown with a linear
  scale that is broken into three segments: the left panel covers
  $\sim$100~Myr, the middle panel covers $\sim$1~Gyr, and the right
  panel covers $\sim$14~Gyr.  The best-fit star formation rate (SFR)
  as a function of age is shown with a thick black line; the
  uncertainty on the fit (including covariance between age bins) is
  shown as a grey shaded envelope.  The distribution of metallicity at
  each age is shown by the mix of colors below the SFR line (Z=0.001
  in blue and downward sloping ; Z=0.0025 in green and upward sloping;
   Z=0.004 in orange and vertical ; Z=0.008 in
 red and horizontal). \label{fig:sfh_lmc} }
\end{figure}

% mass build up
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure12.eps}
\caption{The cumulative stellar mass formed in the the LMC. Shading and colors
same as in previous Figures although the time axis is now linear.
 \label{fig:sfh_cumm} }
\end{figure}


\clearpage

% SFH of the LMC Bar
\begin{figure}[htbp]
\epsfig{figure=figure13a.eps,width=2.9in,angle=0}
\epsfig{figure=figure13b.eps,width=2.9in,angle=0}
\caption{The integrated SFH solutions for the LMC Bar (left) and Outer
  Bar (right) regions.  The shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_bar} }
\end{figure}

% SFH of LMC ``arms''
\begin{figure}[htbp]
\epsfig{figure=figure14a.eps,width=2.9in,angle=0}
\epsfig{figure=figure14b.eps,width=2.9in,angle=0}
\caption{The integrated SFH solutions for the Northwest Arm (left) and
  the Southeast Arm (right) regions.  The shading and colors are the
  same as in Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_arms} }
\end{figure}

% SFH of the ``blue arm'' feature
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure15.eps}
\caption{The integrated SFH solution for the Blue Arm region.  The
  shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_bluearm} }
\end{figure}

% SFH of Constellation III
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure16.eps}
\caption{The integrated SFH solution for the Constellation~III region.
  The shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_consIII} }
\end{figure}

% SFH of 30 Doradus
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure17.eps}
\caption{The integrated SFH solution for the 30~Doradus region.  The
  shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_30dor} }
\end{figure}

% SFH of the Northwest Void
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure18.eps}
\caption{The integrated SFH solution for the Northwest Void region.
  The shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_void} }
\end{figure}

\clearpage

% SFH of the SMC
\begin{figure}[htbp]
\epsscale{0.85}
\plotone{figure19.eps}
\caption{The integrated SFH solution for the Small Magellanic Cloud,
  adapted from \cite{hz04}.  The shading and colors are the same as in
  Figure~\ref{fig:sfh_lmc}. \label{fig:sfh_smc} }
\end{figure}

% Age-metallicity relation derived from the SFH
\begin{figure}[htbp]
\plotone{figure20.eps}
\caption{The Age-Metallicity Relation for the LMC.  The points with
  errorbars are 85 LMC star clusters which have age and metallicity
  measurements in the literature.  The mean metallicity as a function
  of age derived from our SFH analysis is shown as a heavy line, and
  its statistical variance is shown as a grey envelope.  Our analysis
  contains only a single value for ages older than 4~Gyr, because we
  anchored the old SFH to published results based on deep HST
  imaging. \label{fig:agez} }
\end{figure}


==> lmcsfh.tex <==
\begin{deluxetable}{rrrrrrrrrrrrr}
\tabletypesize{\scriptsize}
\tablecolumns{10}
\tablewidth{0pt}
 
\tablecaption{The Star Formation History of the LMC \label{tab:smcsfh}}
\tablehead{
    \colhead{} & \multicolumn{3}{c}{Z = 0.008} & \multicolumn{3}{c}{Z = 0.004} &
        \multicolumn{3}{c}{Z = 0.0025} & \multicolumn{3}{c}{Z = 0.001} \\ 
        \cline{2-4} \cline{5-7} \cline{8-10} \cline{11-13}

    \colhead{log(age)} & 
        \colhead{$SFR$} & \colhead{$SFR_{l}$} & \colhead{$SFR_{u}$} & 
        \colhead{$SFR$} & \colhead{$SFR_{l}$} & \colhead{$SFR_{u}$} & 
        \colhead{$SFR$} & \colhead{$SFR_{l}$} & \colhead{$SFR_{u}$} &
        \colhead{$SFR$} & \colhead{$SFR_{l}$} & \colhead{$SFR_{u}$} 
}
\startdata
\multicolumn{13}{c}{Region AA  ( 04$^h$ 31$^m$,   $-$72\arcdeg\ 17\arcmin )} \\ 
\cline{1-13} 
10.20&0&0&5&0&0&7&0&0&12&39&28&53\\
10.00&0&0&4&0&0&8&0&0&13&24&13&37\\
9.80&0&0&5&0&0&8&0&0&14&17&5&31\\
9.60&0&0&6&0&0&11&0&0&15&0&0&12\\
9.40&0&0&12&67&50&87&191&174&210&14&0&28\\
9.20&0&0&16&0&0&12&0&0&13&0&0&11\\
9.00&4&0&17&0&0&10&0&0&8&0&0&8\\
8.80&7&0&21&0&0&11&0&0&13&17&7&30\\
8.60&0&0&12&11&0&28&0&0&16&0&0&11\\
8.40&0&0&9&0&0&9&0&0&10&0&0&11\\
8.20&0&0&9&0&0&14&0&0&18&10&0&32\\
8.00&0&0&12&0&0&19&9&0&37&5&0&30\\
7.70&8&0&27&0&0&0&0&0&0&0&0&0\\
7.40&12&0&38&0&0&0&0&0&0&0&0&0\\
7.10&0&0&28&0&0&0&0&0&0&0&0&0\\
6.80&0&0&46&0&0&0&0&0&0&0&0&0\\
\enddata
\tablecomments{The complete version of this table is in the 
electronic edition of the Journal. The printed edition contains 
only a sample. SFRs are in units of 10$^{-6} M_\odot {\rm yr}^{-1}$}
\end{deluxetable}

